A Global Physical Model for Cepheids

We perform a global fit to ~5,000 radial velocity and ~177,000 magnitude measurements in 29 photometric bands covering 0.3 to 8.0 microns distributed among 287 Galactic, LMC, and SMC Cepheids with P > 10 days. We assume that the Cepheid light curves and radial velocities are fully characterized by distance, reddening, and time-dependent radius and temperature variations. We construct phase curves of radius and temperature for periods between 10 and 100 days, which yield light curve templates for all our photometric bands and can be easily generalized to any additional band. With only 4 to 6 parameters per Cepheid, depending on the existence of velocity data and the amount of freedom in the distance, the models have typical rms light and velocity curve residuals of 0.05 mag and 3.5 km/s. The model derives the mean Cepheid spectral energy distribution and its derivative with respect to temperature, which deviate from a black body in agreement with metal-line and molecular opacity effects. We determine a mean reddening law towards the Cepheids in our sample, which is not consistent with standard assumptions in either the optical or near-IR. Based on stellar atmosphere models we predict the biases in distance, reddening, and temperature determinations due to the metallicity and we quantify the metallicity signature expected for our fit residuals. The observed residuals as a function of wavelength show clear differences between the individual galaxies, which are compatible with these predictions. In particular, we find that metal-poor Cepheids appear hotter. Finally, we provide a framework for optimally selecting filters that yield the smallest overall errors in Cepheid parameter determination, or filter combinations for suppressing or enhancing the metallicity effects on distance determinations. We make our templates publicly available.

==> galaxy.tex <==
\tablehead{ 
\colhead{Name} & \colhead {$ P$ [d]} & \colhead{$\mu$ [mag]} & \colhead{$E(B-V)$ [mag]} & \colhead{$\bar{v}$ [km s$^{-1}$]} & \colhead{$ \bar{\rho} $} & \colhead{$\bar{\tau}$} & \colhead{$ A^2 \times 10^2$}}
\startdata
         BZ Cyg & 10.1420 & $11.376 \pm 0.040 $ & $0.916 \pm 0.008 $ & \phn $  -11.4 \pm 0.1 $ & $  0.782 \pm 0.008 $ & \phs $  0.032 \pm 0.002 $ & $ 2.2943 \pm 0.0038 $ \\
         SY Aur & 10.1446 & $11.708 \pm 0.040 $ & $0.446 \pm 0.006 $ & \phs \phn \phn $    0.0 \pm 0.1 $ & $  0.723 \pm 0.008 $ & \phs $  0.049 \pm 0.002 $ & $ 2.6711 \pm 0.0047 $ \\
    $\zeta$ Gem & 10.1505 & \phn $ 7.892 \pm 0.025 $ & $-0.031 \pm 0.006 $ & \phs \phn \phn $    6.1 \pm 0.0 $ & $  0.819 \pm 0.005 $ & $ -0.003 \pm 0.002 $ & $ 2.2276 \pm 0.0036 $ \\
         FQ Car & 10.2742 & $13.236 \pm 0.079 $ & $0.597 \pm 0.032 $ & \phn \phn $   -3.7 \pm 0.5 $ & $  0.749 \pm 0.014 $ & $ -0.016 \pm 0.006 $ & $ 3.3464 \pm 0.0044 $ \\
         AN Aur & 10.2893 & $12.981 \pm 0.055 $ & $0.568 \pm 0.008 $ & \phs \phn \phn $    1.9 \pm 0.2 $ & $  0.814 \pm 0.011 $ & \phs $  0.036 \pm 0.002 $ & $ 2.8273 \pm 0.0032 $ \\
          Y Sct & 10.3415 & $11.021 \pm 0.039 $ & $0.735 \pm 0.005 $ & \phs \phn $   14.2 \pm 0.2 $ & $  0.790 \pm 0.008 $ & \phs $  0.000 \pm 0.002 $ & $ 3.3299 \pm 0.0034 $ \\
         MZ Cen & 10.3538 & $13.842 \pm 0.035 $ & $0.665 \pm 0.007 $ & \phn $  -24.4 \pm 0.2 $ & $  0.952 \pm 0.007 $ & $ -0.011 \pm 0.002 $ & $ 2.8914 \pm 0.0047 $ \\
         FO Car & 10.3560 & $13.582 \pm 0.061 $ & $0.380 \pm 0.005 $ & \phn $  -12.1 \pm 0.4 $ & $  0.846 \pm 0.012 $ & \phs $  0.004 \pm 0.002 $ & $ 2.4539 \pm 0.0026 $ \\
         FR Car & 10.7170 & $12.799 \pm 0.016 $ & $0.285 \pm 0.005 $ & \phn \phn $   -6.9 \pm 0.1 $ & $  0.845 \pm 0.003 $ & $ -0.001 \pm 0.002 $ & $ 3.2252 \pm 0.0031 $ \\
         TW Nor & 10.7861 & $11.700 \pm 0.032 $ & $1.090 \pm 0.006 $ & \phn $  -56.1 \pm 0.2 $ & $  0.797 \pm 0.006 $ & $ -0.016 \pm 0.002 $ & $ 3.6645 \pm 0.0034 $ \\
          Z Lac & 10.8857 & $11.291 \pm 0.100 $ & $0.374 \pm 0.003 $ &  \nodata & $  0.803 \pm 0.020 $ & \phs $  0.017 \pm 0.002 $ & $ 3.7122 \pm 0.0028 $ \\
         VX Per & 10.8866 & $12.003 \pm 0.019 $ & $0.484 \pm 0.005 $ & \phn $  -36.3 \pm 0.1 $ & $  0.819 \pm 0.004 $ & \phs $  0.026 \pm 0.002 $ & $ 2.8020 \pm 0.0023 $ \\
         XX Cen & 10.9536 & $10.669 \pm 0.011 $ & $0.238 \pm 0.003 $ & \phn $  -18.1 \pm 0.0 $ & $  0.720 \pm 0.002 $ & \phs $  0.013 \pm 0.002 $ & $ 3.6481 \pm 0.0027 $ \\
         TY Sct & 11.0540 & $11.690 \pm 0.033 $ & $0.927 \pm 0.006 $ & \phs \phn $   25.0 \pm 0.2 $ & $  0.791 \pm 0.006 $ & \phs $  0.007 \pm 0.002 $ & $ 3.6861 \pm 0.0032 $ \\
         SV Per & 11.1292 & $12.520 \pm 0.023 $ & $0.533 \pm 0.006 $ & \phn \phn $   -5.8 \pm 0.1 $ & $  0.913 \pm 0.005 $ & \phs $  0.067 \pm 0.002 $ & $ 3.0448 \pm 0.0029 $ \\
         DR Vel & 11.2013 & $11.314 \pm 0.017 $ & $0.609 \pm 0.005 $ & \phs \phn $   20.5 \pm 0.1 $ & $  0.815 \pm 0.003 $ & $ -0.012 \pm 0.002 $ & $ 3.2269 \pm 0.0032 $ \\
       V438 Cyg & 11.2108 & $11.297 \pm 0.039 $ & $1.111 \pm 0.013 $ & \phn \phn $   -9.1 \pm 0.2 $ & $  0.828 \pm 0.008 $ & $ -0.000 \pm 0.003 $ & $ 3.8962 \pm 0.0048 $ \\
         AD Cam & 11.2622 & $13.878 \pm 0.042 $ & $0.983 \pm 0.012 $ & \phn $  -60.8 \pm 0.2 $ & $  0.826 \pm 0.008 $ & \phs $  0.042 \pm 0.003 $ & $ 3.8923 \pm 0.0047 $ \\
         HZ Per & 11.2796 & $13.844 \pm 0.033 $ & $1.312 \pm 0.012 $ & \phn $  -28.5 \pm 0.2 $ & $  0.896 \pm 0.006 $ & \phs $  0.003 \pm 0.003 $ & $ 3.4095 \pm 0.0044 $ \\
       V340 Nor & 11.2894 & $11.689 \pm 0.061 $ & $0.458 \pm 0.016 $ & \phn $  -40.7 \pm 0.1 $ & $  0.877 \pm 0.012 $ & \phs $  0.043 \pm 0.006 $ & $ 1.3556 \pm 0.0037 $ \\
         AA Gem & 11.3030 & $13.265 \pm 0.017 $ & $0.316 \pm 0.005 $ & \phs \phn $   17.0 \pm 0.1 $ & $  0.905 \pm 0.003 $ & \phs $  0.016 \pm 0.002 $ & $ 2.7887 \pm 0.0028 $ \\
         RX Aur & 11.6235 & $11.090 \pm 0.016 $ & $0.299 \pm 0.005 $ & \phn $  -21.2 \pm 0.1 $ & $  0.826 \pm 0.003 $ & \phs $  0.032 \pm 0.002 $ & $ 2.8715 \pm 0.0023 $ \\
         UU Mus & 11.6362 & $12.551 \pm 0.013 $ & $0.409 \pm 0.003 $ & \phn $  -15.7 \pm 0.1 $ & $  0.821 \pm 0.002 $ & \phs $  0.011 \pm 0.002 $ & $ 4.1536 \pm 0.0035 $ \\
         EZ Cyg & 11.6613 & $13.003 \pm 0.101 $ & $0.570 \pm 0.012 $ & \phs \phn \phn $    2.6 \pm 2.1 $ & $  0.824 \pm 0.020 $ & $ -0.013 \pm 0.003 $ & $ 3.8819 \pm 0.0045 $ \\
         RY Cas & 12.1384 & $11.880 \pm 0.020 $ & $0.606 \pm 0.007 $ & \phn $  -84.2 \pm 0.1 $ & $  0.775 \pm 0.004 $ & \phs $  0.014 \pm 0.002 $ & $ 3.9806 \pm 0.0043 $ \\
         KK Cen & 12.1820 & $13.775 \pm 0.062 $ & $0.597 \pm 0.005 $ & \phn \phn $   -2.3 \pm 0.3 $ & $  0.827 \pm 0.012 $ & \phs $  0.020 \pm 0.002 $ & $ 4.2655 \pm 0.0041 $ \\
         VX Cru & 12.2131 & $12.632 \pm 0.042 $ & $0.860 \pm 0.006 $ & \phn $  -25.8 \pm 0.2 $ & $  0.707 \pm 0.008 $ & \phs $  0.007 \pm 0.002 $ & $ 4.0726 \pm 0.0038 $ \\
         AS Vul & 12.2255 & $12.899 \pm 0.101 $ & $0.968 \pm 0.011 $ &  \nodata & $  0.838 \pm 0.020 $ & $ -0.017 \pm 0.003 $ & $ 3.9987 \pm 0.0042 $ \\
         SS CMa & 12.3563 & $12.553 \pm 0.100 $ & $0.524 \pm 0.004 $ &  \nodata & $  0.841 \pm 0.020 $ & \phs $  0.020 \pm 0.002 $ & $ 3.8946 \pm 0.0028 $ \\
         XY Car & 12.4358 & $11.999 \pm 0.013 $ & $0.340 \pm 0.005 $ & \phn \phn $   -5.7 \pm 0.0 $ & $  0.811 \pm 0.002 $ & $ -0.008 \pm 0.002 $ & $ 4.0850 \pm 0.0033 $ \\
          U Nor & 12.6443 & $10.226 \pm 0.015 $ & $0.836 \pm 0.005 $ & \phn $  -21.7 \pm 0.1 $ & $  0.745 \pm 0.003 $ & \phs $  0.011 \pm 0.002 $ & $ 4.4978 \pm 0.0041 $ \\
         GQ Vul & 12.6455 & $12.918 \pm 0.102 $ & $1.670 \pm 0.025 $ &  \nodata & $  0.848 \pm 0.020 $ & \phs $  0.051 \pm 0.005 $ & $ 4.0893 \pm 0.0064 $ \\
         SU Cru & 12.8490 & \phn $ 9.614 \pm 0.018 $ & $1.066 \pm 0.006 $ & \phn $  -28.5 \pm 0.0 $ & $  0.657 \pm 0.003 $ & \phs $  0.016 \pm 0.002 $ & $ 3.6537 \pm 0.0027 $ \\
         OO Cen & 12.8827 & $13.180 \pm 0.041 $ & $0.869 \pm 0.006 $ & \phn $  -33.0 \pm 0.2 $ & $  0.892 \pm 0.008 $ & $ -0.022 \pm 0.002 $ & $ 4.1778 \pm 0.0058 $ \\
         GX Sge & 12.9001 & $12.735 \pm 0.101 $ & $1.118 \pm 0.012 $ &  \nodata & $  0.854 \pm 0.020 $ & $ -0.015 \pm 0.003 $ & $ 4.9561 \pm 0.0048 $ \\
          Z Sct & 12.9022 & $12.073 \pm 0.039 $ & $0.457 \pm 0.004 $ & \phs \phn $   27.9 \pm 0.2 $ & $  0.864 \pm 0.008 $ & $ -0.016 \pm 0.002 $ & $ 4.9233 \pm 0.0038 $ \\
      V1364 Cyg & 12.9727 & $13.678 \pm 0.101 $ & $1.112 \pm 0.016 $ &  \nodata & $  0.856 \pm 0.020 $ & $ -0.005 \pm 0.004 $ & $ 3.8260 \pm 0.0043 $ \\
         IO Car & 13.1061 & $13.085 \pm 0.069 $ & $0.616 \pm 0.009 $ & \phs \phn $   29.1 \pm 0.1 $ & $  0.705 \pm 0.014 $ & \phs $  0.050 \pm 0.003 $ & $ 1.6402 \pm 0.0045 $ \\
         EX Vel & 13.2338 & $13.517 \pm 0.057 $ & $0.740 \pm 0.006 $ & \phs \phn $   32.5 \pm 0.5 $ & $  0.898 \pm 0.011 $ & \phs $  0.002 \pm 0.002 $ & $ 3.7759 \pm 0.0043 $ \\
       V916 Aql & 13.4417 & $12.320 \pm 0.022 $ & $0.692 \pm 0.008 $ & \phs \phn $   17.9 \pm 0.1 $ & $  0.899 \pm 0.004 $ & $ -0.045 \pm 0.002 $ & $ 4.4975 \pm 0.0039 $ \\
         HW Pup & 13.4564 & $14.340 \pm 0.037 $ & $0.682 \pm 0.006 $ & \phs $  115.4 \pm 0.2 $ & $  0.811 \pm 0.007 $ & \phs $  0.045 \pm 0.002 $ & $ 4.5434 \pm 0.0042 $ \\
         FI Car & 13.4566 & $13.736 \pm 0.037 $ & $0.746 \pm 0.006 $ & \phs \phn $   13.0 \pm 0.2 $ & $  0.923 \pm 0.007 $ & \phs $  0.008 \pm 0.002 $ & $ 3.6456 \pm 0.0033 $ \\
         VY Sgr & 13.5586 & $11.675 \pm 0.046 $ & $1.134 \pm 0.008 $ & \phs \phn $   14.7 \pm 0.3 $ & $  0.840 \pm 0.009 $ & $ -0.011 \pm 0.002 $ & $ 5.0622 \pm 0.0039 $ \\
         AD Pup & 13.5964 & $13.269 \pm 0.100 $ & $0.298 \pm 0.004 $ &  \nodata & $  0.870 \pm 0.020 $ & \phs $  0.011 \pm 0.002 $ & $ 4.8289 \pm 0.0036 $ \\
         DG Vul & 13.6083 & $11.543 \pm 0.049 $ & $1.027 \pm 0.010 $ & \phs \phn \phn $    1.9 \pm 0.3 $ & $  0.794 \pm 0.010 $ & $ -0.024 \pm 0.003 $ & $ 4.6594 \pm 0.0040 $ \\
         SZ Cas & 13.6370 & $11.559 \pm 0.087 $ & $0.806 \pm 0.006 $ & \phn $  -46.5 \pm 0.4 $ & $  0.810 \pm 0.017 $ & \phs $  0.036 \pm 0.002 $ & $ 2.0063 \pm 0.0016 $ \\
         BN Pup & 13.6723 & $12.945 \pm 0.011 $ & $0.394 \pm 0.003 $ & \phs \phn $   62.3 \pm 0.1 $ & $  0.891 \pm 0.002 $ & $ -0.000 \pm 0.002 $ & $ 5.1221 \pm 0.0040 $ \\
         TT Aql & 13.7551 & \phn $ 9.874 \pm 0.010 $ & $0.398 \pm 0.003 $ & \phs \phn \phn $    3.0 \pm 0.0 $ & $  0.876 \pm 0.002 $ & $ -0.018 \pm 0.002 $ & $ 4.7939 \pm 0.0038 $ \\
         CY Aur & 13.8465 & $14.262 \pm 0.028 $ & $0.834 \pm 0.010 $ & \phn $  -13.3 \pm 0.2 $ & $  1.003 \pm 0.005 $ & \phs $  0.020 \pm 0.002 $ & $ 3.8275 \pm 0.0044 $ \\
         SV Vel & 14.0976 & $11.261 \pm 0.018 $ & $0.362 \pm 0.004 $ & \phs \phn \phn $    4.2 \pm 0.1 $ & $  0.775 \pm 0.003 $ & \phs $  0.008 \pm 0.002 $ & $ 4.7354 \pm 0.0038 $ \\
         LS Pup & 14.1479 & $13.745 \pm 0.015 $ & $0.445 \pm 0.004 $ & \phs \phn $   77.4 \pm 0.1 $ & $  0.965 \pm 0.003 $ & \phs $  0.004 \pm 0.002 $ & $ 4.1883 \pm 0.0039 $ \\
         CY Cas & 14.3789 & $13.006 \pm 0.101 $ & $0.985 \pm 0.010 $ &  \nodata & $  0.887 \pm 0.020 $ & \phs $  0.021 \pm 0.003 $ & $ 5.3735 \pm 0.0069 $ \\
         TX Cyg & 14.7101 & $10.283 \pm 0.100 $ & $1.136 \pm 0.007 $ &  \nodata & $  0.894 \pm 0.020 $ & \phs $  0.015 \pm 0.002 $ & $ 5.2606 \pm 0.0048 $ \\
         UZ Sct & 14.7482 & $12.444 \pm 0.029 $ & $0.996 \pm 0.009 $ & \phs \phn $   38.2 \pm 0.1 $ & $  0.933 \pm 0.006 $ & $ -0.006 \pm 0.002 $ & $ 4.0855 \pm 0.0036 $ \\
         RW Cas & 14.7917 & $12.269 \pm 0.013 $ & $0.353 \pm 0.005 $ & \phn $  -71.6 \pm 0.1 $ & $  0.897 \pm 0.002 $ & $ -0.014 \pm 0.002 $ & $ 5.3241 \pm 0.0043 $ \\
         VW Cen & 15.0374 & $12.771 \pm 0.012 $ & $0.450 \pm 0.003 $ & \phn $  -29.9 \pm 0.1 $ & $  0.893 \pm 0.002 $ & $ -0.026 \pm 0.002 $ & $ 5.3053 \pm 0.0044 $ \\
         CH Cas & 15.0885 & $12.194 \pm 0.072 $ & $0.999 \pm 0.009 $ & \phn $  -55.9 \pm 0.5 $ & $  0.840 \pm 0.014 $ & \phs $  0.031 \pm 0.002 $ & $ 4.9112 \pm 0.0051 $ \\
         SZ Cyg & 15.1103 & $11.857 \pm 0.017 $ & $0.545 \pm 0.005 $ & \phn $  -11.2 \pm 0.1 $ & $  0.932 \pm 0.003 $ & $ -0.024 \pm 0.002 $ & $ 4.4713 \pm 0.0041 $ \\
         SV Mon & 15.2334 & $11.899 \pm 0.011 $ & $0.194 \pm 0.004 $ & \phs \phn $   27.6 \pm 0.0 $ & $  0.906 \pm 0.002 $ & $ -0.011 \pm 0.002 $ & $ 5.3500 \pm 0.0047 $ \\
         AV Sgr & 15.4107 & $11.376 \pm 0.041 $ & $1.202 \pm 0.009 $ & \phs \phn $   17.9 \pm 0.4 $ & $  0.868 \pm 0.008 $ & $ -0.017 \pm 0.002 $ & $ 5.6320 \pm 0.0052 $ \\
         ER Aur & 15.6983 & $14.738 \pm 0.101 $ & $0.637 \pm 0.009 $ &  \nodata & $  0.914 \pm 0.020 $ & \phs $  0.069 \pm 0.002 $ & $ 2.9403 \pm 0.0028 $ \\
         XX Car & 15.7097 & $12.297 \pm 0.010 $ & $0.320 \pm 0.004 $ & \phn $  -11.4 \pm 0.0 $ & $  0.811 \pm 0.002 $ & \phs $  0.005 \pm 0.002 $ & $ 5.7070 \pm 0.0040 $ \\
       V470 Sco & 16.2611 & $10.445 \pm 0.069 $ & $1.556 \pm 0.010 $ & \phn \phn $   -3.4 \pm 0.5 $ & $  0.883 \pm 0.014 $ & \phs $  0.022 \pm 0.003 $ & $ 4.5236 \pm 0.0045 $ \\
          X Cyg & 16.3860 & \phn $ 9.929 \pm 0.009 $ & $0.192 \pm 0.003 $ & \phs \phn \phn $    7.7 \pm 0.0 $ & $  0.923 \pm 0.002 $ & $ -0.026 \pm 0.002 $ & $ 5.4327 \pm 0.0040 $ \\
         RW Cam & 16.4154 & $11.713 \pm 0.077 $ & $0.792 \pm 0.006 $ & \phn $  -25.0 \pm 0.7 $ & $  0.997 \pm 0.015 $ & \phs $  0.061 \pm 0.002 $ & $ 3.6379 \pm 0.0029 $ \\
         XZ Car & 16.6523 & $11.720 \pm 0.011 $ & $0.318 \pm 0.004 $ & \phs \phn \phn $    1.5 \pm 0.0 $ & $  0.917 \pm 0.002 $ & $ -0.023 \pm 0.002 $ & $ 5.4409 \pm 0.0040 $ \\
         CD Cyg & 17.0742 & $11.844 \pm 0.011 $ & $0.439 \pm 0.004 $ & \phn $  -12.5 \pm 0.1 $ & $  0.936 \pm 0.002 $ & $ -0.019 \pm 0.002 $ & $ 5.8261 \pm 0.0043 $ \\
         TX Cen & 17.0971 & $12.816 \pm 0.016 $ & $0.805 \pm 0.006 $ & \phn $  -51.6 \pm 0.1 $ & $  1.060 \pm 0.003 $ & $ -0.020 \pm 0.002 $ & $ 5.4023 \pm 0.0042 $ \\
          Y Oph & 17.1254 & \phn $ 8.143 \pm 0.014 $ & $0.594 \pm 0.004 $ & \phn \phn $   -7.2 \pm 0.0 $ & $  0.792 \pm 0.003 $ & \phs $  0.011 \pm 0.002 $ & $ 2.5844 \pm 0.0014 $ \\
         SZ Aql & 17.1395 & $11.187 \pm 0.015 $ & $0.480 \pm 0.003 $ & \phs \phn \phn $    7.0 \pm 0.1 $ & $  0.925 \pm 0.003 $ & $ -0.031 \pm 0.002 $ & $ 5.8809 \pm 0.0043 $ \\
         AA Ser & 17.1421 & $12.265 \pm 0.074 $ & $1.207 \pm 0.010 $ & \phn $  -45.4 \pm 0.6 $ & $  0.961 \pm 0.015 $ & $ -0.052 \pm 0.003 $ & $ 4.3670 \pm 0.0041 $ \\
         QY Cen & 17.7518 & $12.278 \pm 0.039 $ & $1.059 \pm 0.008 $ & \phn $  -59.0 \pm 0.3 $ & $  0.959 \pm 0.008 $ & $ -0.054 \pm 0.002 $ & $ 5.2747 \pm 0.0056 $ \\
         CP Cep & 17.8636 & $13.054 \pm 0.019 $ & $0.675 \pm 0.009 $ & \phn $  -40.7 \pm 0.1 $ & $  1.029 \pm 0.003 $ & $ -0.025 \pm 0.002 $ & $ 3.9504 \pm 0.0035 $ \\
         YZ Car & 18.1653 & $12.289 \pm 0.100 $ & $0.371 \pm 0.004 $ &  \nodata & $  0.958 \pm 0.020 $ & \phs $  0.011 \pm 0.002 $ & $ 4.0286 \pm 0.0028 $ \\
         YZ Aur & 18.1927 & $13.694 \pm 0.018 $ & $0.714 \pm 0.009 $ & \phn $  -12.1 \pm 0.1 $ & $  1.075 \pm 0.003 $ & \phs $  0.034 \pm 0.002 $ & $ 4.1407 \pm 0.0036 $ \\
         RU Sct & 19.7041 & $11.233 \pm 0.013 $ & $0.843 \pm 0.005 $ & \phn \phn $   -4.9 \pm 0.1 $ & $  0.959 \pm 0.002 $ & $ -0.011 \pm 0.002 $ & $ 5.3616 \pm 0.0044 $ \\
         KX Cyg & 20.0539 & $11.718 \pm 0.101 $ & $1.538 \pm 0.012 $ &  \nodata & $  0.988 \pm 0.020 $ & \phs $  0.001 \pm 0.003 $ & $ 5.3064 \pm 0.0054 $ \\
         VX Cyg & 20.1333 & $12.342 \pm 0.017 $ & $0.833 \pm 0.007 $ & \phn $  -16.4 \pm 0.1 $ & $  1.042 \pm 0.003 $ & $ -0.006 \pm 0.002 $ & $ 4.9277 \pm 0.0047 $ \\
         RY Sco & 20.3209 & $10.154 \pm 0.013 $ & $0.725 \pm 0.004 $ & \phn $  -18.3 \pm 0.0 $ & $  0.896 \pm 0.002 $ & \phs $  0.015 \pm 0.002 $ & $ 3.9600 \pm 0.0030 $ \\
         RZ Vel & 20.3991 & $10.701 \pm 0.009 $ & $0.292 \pm 0.003 $ & \phs \phn $   24.9 \pm 0.0 $ & $  0.975 \pm 0.002 $ & $ -0.017 \pm 0.002 $ & $ 6.2352 \pm 0.0050 $ \\
       V340 Ara & 20.8092 & $12.845 \pm 0.041 $ & $0.367 \pm 0.006 $ & \phn $  -83.3 \pm 0.3 $ & $  1.000 \pm 0.008 $ & $ -0.081 \pm 0.002 $ & $ 5.7942 \pm 0.0050 $ \\
         IY Cyg & 21.7599 & $14.341 \pm 0.101 $ & $1.234 \pm 0.013 $ &  \nodata & $  1.013 \pm 0.020 $ & \phs $  0.027 \pm 0.003 $ & $ 5.8267 \pm 0.0060 $ \\
         WZ Sgr & 21.8508 & $11.070 \pm 0.009 $ & $0.441 \pm 0.003 $ & \phn $  -17.9 \pm 0.0 $ & $  1.010 \pm 0.002 $ & $ -0.036 \pm 0.002 $ & $ 5.7456 \pm 0.0039 $ \\
         BM Per & 22.9565 & $12.271 \pm 0.020 $ & $0.825 \pm 0.008 $ & \phn $  -43.1 \pm 0.1 $ & $  1.032 \pm 0.004 $ & $ -0.037 \pm 0.002 $ & $ 6.3738 \pm 0.0054 $ \\
         WZ Car & 23.0159 & $12.825 \pm 0.009 $ & $0.390 \pm 0.003 $ & \phn $  -15.1 \pm 0.0 $ & $  0.992 \pm 0.001 $ & $ -0.003 \pm 0.002 $ & $ 6.6248 \pm 0.0046 $ \\
         VZ Pup & 23.1746 & $13.150 \pm 0.009 $ & $0.412 \pm 0.003 $ & \phs \phn $   63.0 \pm 0.0 $ & $  0.981 \pm 0.002 $ & \phs $  0.005 \pm 0.002 $ & $ 6.4050 \pm 0.0044 $ \\
         SW Vel & 23.4281 & $11.812 \pm 0.009 $ & $0.342 \pm 0.004 $ & \phs \phn $   22.7 \pm 0.0 $ & $  1.005 \pm 0.002 $ & $ -0.010 \pm 0.002 $ & $ 6.5808 \pm 0.0047 $ \\
          X Pup & 25.9674 & $12.581 \pm 0.015 $ & $0.420 \pm 0.003 $ & \phs \phn $   65.6 \pm 0.2 $ & $  1.123 \pm 0.003 $ & $ -0.008 \pm 0.002 $ & $ 6.8403 \pm 0.0052 $ \\
          T Mon & 27.0299 & $10.451 \pm 0.008 $ & $0.173 \pm 0.003 $ & \phs \phn $   22.7 \pm 0.0 $ & $  1.085 \pm 0.001 $ & $ -0.034 \pm 0.002 $ & $ 5.6955 \pm 0.0035 $ \\
         RY Vel & 28.1238 & $11.421 \pm 0.012 $ & $0.551 \pm 0.004 $ & \phn $  -10.4 \pm 0.0 $ & $  0.994 \pm 0.002 $ & $ -0.000 \pm 0.002 $ & $ 5.2871 \pm 0.0046 $ \\
         KQ Sco & 28.6915 & $11.813 \pm 0.014 $ & $0.839 \pm 0.005 $ & \phn $  -24.1 \pm 0.1 $ & $  1.123 \pm 0.002 $ & $ -0.057 \pm 0.002 $ & $ 5.5869 \pm 0.0052 $ \\
         AQ Pup & 30.1060 & $12.217 \pm 0.009 $ & $0.430 \pm 0.004 $ & \phs \phn $   56.9 \pm 0.0 $ & $  1.097 \pm 0.002 $ & $ -0.032 \pm 0.002 $ & $ 6.8331 \pm 0.0051 $ \\
       V609 Cyg & 31.0806 & $12.621 \pm 0.101 $ & $1.068 \pm 0.008 $ &  \nodata & $  1.121 \pm 0.020 $ & $ -0.029 \pm 0.002 $ & $ 6.5599 \pm 0.0055 $ \\
       V396 Cyg & 33.2482 & $11.974 \pm 0.101 $ & $1.717 \pm 0.011 $ &  \nodata & $  1.141 \pm 0.020 $ & \phs $  0.049 \pm 0.003 $ & $ 5.2302 \pm 0.0042 $ \\
         EZ Vel & 34.5507 & $14.931 \pm 0.043 $ & $0.884 \pm 0.007 $ & \phs \phn $   94.7 \pm 0.3 $ & $  1.143 \pm 0.009 $ & $ -0.017 \pm 0.002 $ & $ 6.0125 \pm 0.0053 $ \\
     $\ell$ Car & 35.5466 & \phn $ 8.291 \pm 0.009 $ & $0.115 \pm 0.003 $ & \phs \phn \phn $    2.5 \pm 0.0 $ & $  1.164 \pm 0.002 $ & $ -0.059 \pm 0.002 $ & $ 4.5772 \pm 0.0029 $ \\
          U Car & 38.8210 & $10.570 \pm 0.009 $ & $0.234 \pm 0.003 $ & \phs \phn \phn $    2.1 \pm 0.0 $ & $  1.119 \pm 0.002 $ & $ -0.035 \pm 0.002 $ & $ 6.4117 \pm 0.0050 $ \\
      V1467 Cyg & 48.5054 & $14.246 \pm 0.101 $ & $1.571 \pm 0.010 $ &  \nodata & $  1.256 \pm 0.020 $ & $ -0.017 \pm 0.003 $ & $ 5.5179 \pm 0.0049 $ \\
\enddata


==> lmc.tex <==
\tablehead{ 
\colhead{Name} & \colhead {$ P$ [d]} & \colhead{$\mu$ [mag]} & \colhead{$E(B-V)$ [mag]} & \colhead{$\bar{v}$ [km s$^{-1}$]} & \colhead{$ \bar{\rho} $} & \colhead{$\bar{\tau}$} & \colhead{$ A^2 \times 10^2$}}
\startdata
       HV 01016 & 10.0438 & 18.480 & $0.147 \pm 0.019 $ &  \nodata & $  0.761 \pm 0.003 $ & \phs $  0.025 \pm 0.006 $ & $ 2.6563 \pm 0.0067 $ \\
      OIII 2562 & 10.0716 & 18.479 & $0.147 \pm 0.019 $ &  \nodata & $  0.788 \pm 0.003 $ & \phs $  0.033 \pm 0.006 $ & $ 0.9424 \pm 0.0018 $ \\
       HV 00923 & 10.2547 & 18.511 & $0.144 \pm 0.019 $ &  \nodata & $  0.784 \pm 0.002 $ & \phs $  0.039 \pm 0.006 $ & $ 2.3734 \pm 0.0030 $ \\
      OIII 0057 & 10.3075 & 18.558 & $0.150 \pm 0.019 $ &  \nodata & $  0.809 \pm 0.003 $ & \phs $  0.027 \pm 0.006 $ & $ 2.0783 \pm 0.0033 $ \\
       HV 02371 & 10.3479 & 18.514 & $0.142 \pm 0.019 $ &  \nodata & $  0.780 \pm 0.003 $ & \phs $  0.046 \pm 0.006 $ & $ 3.3251 \pm 0.0042 $ \\
      OIII 0114 & 10.3727 & 18.552 & $0.142 \pm 0.019 $ &  \nodata & $  0.789 \pm 0.003 $ & \phs $  0.048 \pm 0.006 $ & $ 2.5954 \pm 0.0040 $ \\
       HV 02277 & 10.4135 & 18.533 & $0.142 \pm 0.019 $ &  \nodata & $  0.798 \pm 0.003 $ & \phs $  0.051 \pm 0.006 $ & $ 3.4945 \pm 0.0050 $ \\
      OIII 3284 & 10.4772 & 18.447 & $0.147 \pm 0.019 $ &  \nodata & $  0.774 \pm 0.003 $ & \phs $  0.025 \pm 0.006 $ & $ 2.3392 \pm 0.0043 $ \\
       HV 05551 & 10.4852 & 18.544 & $0.093 \pm 0.011 $ &  \nodata & $  0.777 \pm 0.001 $ & \phs $  0.016 \pm 0.003 $ & $ 2.0011 \pm 0.0033 $ \\
       HV 13064 & 10.4872 & 18.482 & $0.191 \pm 0.019 $ &  \nodata & $  0.841 \pm 0.003 $ & $ -0.099 \pm 0.006 $ & $ 3.0641 \pm 0.0056 $ \\
      OIII 0016 & 10.5070 & 18.554 & $0.169 \pm 0.019 $ &  \nodata & $  0.905 \pm 0.003 $ & $ -0.004 \pm 0.006 $ & $ 0.6998 \pm 0.0018 $ \\
      OIII 0978 & 10.5199 & 18.517 & $0.157 \pm 0.019 $ &  \nodata & $  0.840 \pm 0.003 $ & \phs $  0.013 \pm 0.006 $ & $ 1.7861 \pm 0.0027 $ \\
      OIII 1784 & 10.6628 & 18.492 & $0.147 \pm 0.019 $ &  \nodata & $  0.777 \pm 0.003 $ & \phs $  0.023 \pm 0.006 $ & $ 2.9994 \pm 0.0042 $ \\
       HV 12078 & 10.6876 & 18.427 & $0.088 \pm 0.010 $ &  \nodata & $  0.802 \pm 0.001 $ & \phs $  0.004 \pm 0.003 $ & $ 2.0235 \pm 0.0030 $ \\
      OIII 0798 & 10.7104 & 18.526 & $0.145 \pm 0.019 $ &  \nodata & $  0.789 \pm 0.003 $ & \phs $  0.032 \pm 0.006 $ & $ 1.7056 \pm 0.0023 $ \\
       HV 12537 & 10.7923 & 18.531 & $0.142 \pm 0.019 $ &  \nodata & $  0.819 \pm 0.003 $ & \phs $  0.053 \pm 0.006 $ & $ 3.2753 \pm 0.0037 $ \\
       HV 02280 & 10.8548 & 18.525 & $0.143 \pm 0.019 $ &  \nodata & $  0.801 \pm 0.003 $ & \phs $  0.041 \pm 0.006 $ & $ 2.9274 \pm 0.0032 $ \\
       HV 02432 & 10.9192 & 18.494 & $0.247 \pm 0.010 $ &  \nodata & $  0.787 \pm 0.002 $ & \phs $  0.100 \pm 0.004 $ & $ 2.9310 \pm 0.0037 $ \\
       HV 02864 & 10.9853 & 18.426 & $0.095 \pm 0.006 $ & \phs $  259.8 \pm 0.1 $ & $  0.791 \pm 0.001 $ & \phs $  0.020 \pm 0.002 $ & $ 3.7166 \pm 0.0037 $ \\
       HV 02598 & 10.9913 & 18.486 & $0.138 \pm 0.019 $ &  \nodata & $  0.806 \pm 0.003 $ & \phs $  0.060 \pm 0.006 $ & $ 2.1020 \pm 0.0020 $ \\
       HV 00921 & 11.0905 & 18.506 & $0.147 \pm 0.019 $ &  \nodata & $  0.811 \pm 0.003 $ & \phs $  0.030 \pm 0.006 $ & $ 2.1498 \pm 0.0024 $ \\
       HV 00999 & 11.2318 & 18.461 & $0.147 \pm 0.019 $ &  \nodata & $  0.823 \pm 0.003 $ & \phs $  0.033 \pm 0.006 $ & $ 2.7614 \pm 0.0035 $ \\
      OIII 2911 & 11.2404 & 18.456 & $0.127 \pm 0.019 $ &  \nodata & $  0.756 \pm 0.003 $ & \phs $  0.075 \pm 0.006 $ & $ 0.9602 \pm 0.0015 $ \\
       HV 02462 & 11.2459 & 18.512 & $0.150 \pm 0.019 $ &  \nodata & $  0.800 \pm 0.003 $ & \phs $  0.013 \pm 0.006 $ & $ 3.7851 \pm 0.0054 $ \\
       HV 12716 & 11.2554 & 18.581 & $0.150 \pm 0.019 $ &  \nodata & $  0.842 \pm 0.003 $ & \phs $  0.028 \pm 0.006 $ & $ 3.1213 \pm 0.0047 $ \\
       HV 02585 & 11.2627 & 18.486 & $0.145 \pm 0.019 $ &  \nodata & $  0.797 \pm 0.003 $ & \phs $  0.029 \pm 0.006 $ & $ 2.7015 \pm 0.0036 $ \\
       HV 02787 & 11.4463 & 18.463 & $0.138 \pm 0.019 $ &  \nodata & $  0.784 \pm 0.003 $ & \phs $  0.045 \pm 0.006 $ & $ 3.7997 \pm 0.0049 $ \\
       HV 05979 & 11.5317 & 18.480 & $0.158 \pm 0.019 $ &  \nodata & $  0.818 \pm 0.003 $ & $ -0.009 \pm 0.006 $ & $ 2.1086 \pm 0.0025 $ \\
       HV 00880 & 11.6710 & 18.520 & $0.132 \pm 0.019 $ &  \nodata & $  0.792 \pm 0.003 $ & \phs $  0.067 \pm 0.006 $ & $ 3.5703 \pm 0.0046 $ \\
      OIII 3163 & 11.8367 & 18.440 & $0.153 \pm 0.019 $ &  \nodata & $  0.854 \pm 0.003 $ & \phs $  0.015 \pm 0.006 $ & $ 2.0637 \pm 0.0035 $ \\
       HV 00905 & 11.8602 & 18.514 & $0.142 \pm 0.019 $ &  \nodata & $  0.826 \pm 0.002 $ & \phs $  0.043 \pm 0.006 $ & $ 3.9445 \pm 0.0047 $ \\
       HV 00906 & 11.9049 & 18.515 & $0.148 \pm 0.019 $ &  \nodata & $  0.836 \pm 0.003 $ & \phs $  0.026 \pm 0.006 $ & $ 3.4683 \pm 0.0044 $ \\
       HV 02299 & 12.0652 & 18.506 & $0.146 \pm 0.019 $ &  \nodata & $  0.866 \pm 0.003 $ & \phs $  0.042 \pm 0.006 $ & $ 3.5988 \pm 0.0056 $ \\
       HV 02815 & 12.0899 & 18.460 & $0.152 \pm 0.019 $ &  \nodata & $  0.831 \pm 0.003 $ & \phs $  0.009 \pm 0.006 $ & $ 3.4912 \pm 0.0054 $ \\
      OIII 0716 & 12.1886 & 18.528 & $0.149 \pm 0.019 $ &  \nodata & $  0.820 \pm 0.003 $ & \phs $  0.014 \pm 0.006 $ & $ 3.5748 \pm 0.0041 $ \\
       HV 12519 & 12.1956 & 18.511 & $0.145 \pm 0.019 $ &  \nodata & $  0.835 \pm 0.003 $ & \phs $  0.032 \pm 0.006 $ & $ 2.9309 \pm 0.0041 $ \\
      OIII 0812 & 12.1957 & 18.527 & $0.146 \pm 0.019 $ &  \nodata & $  0.836 \pm 0.003 $ & \phs $  0.028 \pm 0.006 $ & $ 3.7183 \pm 0.0043 $ \\
       HV 00978 & 12.2634 & 18.494 & $0.146 \pm 0.019 $ &  \nodata & $  0.837 \pm 0.003 $ & \phs $  0.029 \pm 0.006 $ & $ 2.9271 \pm 0.0030 $ \\
       HV 12475 & 12.3269 & 18.544 & $0.149 \pm 0.019 $ &  \nodata & $  0.831 \pm 0.003 $ & \phs $  0.014 \pm 0.006 $ & $ 4.1995 \pm 0.0053 $ \\
       HV 00958 & 12.3596 & 18.498 & $0.149 \pm 0.019 $ &  \nodata & $  0.838 \pm 0.003 $ & \phs $  0.017 \pm 0.006 $ & $ 3.4571 \pm 0.0033 $ \\
      OIII 0167 & 12.5118 & 18.548 & $0.144 \pm 0.019 $ &  \nodata & $  0.850 \pm 0.003 $ & \phs $  0.038 \pm 0.006 $ & $ 2.7968 \pm 0.0043 $ \\
       HV 00898 & 12.6206 & 18.516 & $0.145 \pm 0.019 $ &  \nodata & $  0.838 \pm 0.003 $ & \phs $  0.029 \pm 0.006 $ & $ 3.7199 \pm 0.0047 $ \\
       HV 02285 & 12.6361 & 18.524 & $0.139 \pm 0.019 $ &  \nodata & $  0.823 \pm 0.003 $ & \phs $  0.042 \pm 0.006 $ & $ 4.5599 \pm 0.0057 $ \\
       HV 00874 & 12.6828 & 18.554 & $0.089 \pm 0.009 $ &  \nodata & $  0.838 \pm 0.001 $ & \phs $  0.022 \pm 0.003 $ & $ 5.0806 \pm 0.0061 $ \\
       HV 02321 & 12.7218 & 18.517 & $0.148 \pm 0.019 $ &  \nodata & $  0.852 \pm 0.003 $ & \phs $  0.021 \pm 0.006 $ & $ 4.1784 \pm 0.0048 $ \\
       HV 12839 & 12.7704 & 18.497 & $0.136 \pm 0.019 $ &  \nodata & $  0.823 \pm 0.003 $ & \phs $  0.050 \pm 0.006 $ & $ 4.7680 \pm 0.0066 $ \\
       HV 00895 & 12.9165 & 18.518 & $0.136 \pm 0.019 $ &  \nodata & $  0.817 \pm 0.003 $ & \phs $  0.047 \pm 0.006 $ & $ 5.1729 \pm 0.0056 $ \\
       HV 02527 & 12.9494 & 18.512 & $0.104 \pm 0.007 $ &  \nodata & $  0.860 \pm 0.002 $ & \phs $  0.005 \pm 0.003 $ & $ 4.8937 \pm 0.0062 $ \\
       HV 02260 & 12.9878 & 18.524 & $0.218 \pm 0.006 $ &  \nodata & $  0.807 \pm 0.001 $ & \phs $  0.034 \pm 0.002 $ & $ 4.6207 \pm 0.0056 $ \\
      OIII 1862 & 13.1249 & 18.496 & $0.149 \pm 0.019 $ &  \nodata & $  0.843 \pm 0.003 $ & \phs $  0.013 \pm 0.006 $ & $ 3.7787 \pm 0.0051 $ \\
       HV 00997 & 13.1436 & 18.467 & $0.211 \pm 0.006 $ &  \nodata & $  0.857 \pm 0.001 $ & \phs $  0.032 \pm 0.002 $ & $ 4.7540 \pm 0.0070 $ \\
       HV 00932 & 13.2834 & 18.506 & $0.185 \pm 0.010 $ &  \nodata & $  0.857 \pm 0.002 $ & \phs $  0.058 \pm 0.004 $ & $ 5.2969 \pm 0.0067 $ \\
       HV 12656 & 13.4003 & 18.478 & $0.105 \pm 0.011 $ &  \nodata & $  0.873 \pm 0.003 $ & \phs $  0.034 \pm 0.004 $ & $ 2.7095 \pm 0.0045 $ \\
      OIII 1539 & 13.5129 & 18.505 & $0.149 \pm 0.019 $ &  \nodata & $  0.877 \pm 0.003 $ & \phs $  0.021 \pm 0.006 $ & $ 3.8818 \pm 0.0036 $ \\
       HV 02270 & 13.6262 & 18.537 & $0.208 \pm 0.010 $ &  \nodata & $  0.856 \pm 0.002 $ & \phs $  0.033 \pm 0.003 $ & $ 3.7819 \pm 0.0037 $ \\
       HV 02352 & 13.6307 & 18.532 & $0.172 \pm 0.007 $ &  \nodata & $  0.875 \pm 0.002 $ & \phs $  0.053 \pm 0.002 $ & $ 3.2582 \pm 0.0053 $ \\
      OIII 3091 & 13.6406 & 18.450 & $0.160 \pm 0.019 $ &  \nodata & $  0.905 \pm 0.003 $ & $ -0.008 \pm 0.006 $ & $ 2.3246 \pm 0.0035 $ \\
       HV 01019 & 13.6597 & 18.472 & $0.298 \pm 0.009 $ &  \nodata & $  0.836 \pm 0.002 $ & \phs $  0.081 \pm 0.003 $ & $ 2.8520 \pm 0.0026 $ \\
       HV 12724 & 13.7456 & 18.563 & $0.144 \pm 0.011 $ &  \nodata & $  0.880 \pm 0.002 $ & \phs $  0.000 \pm 0.004 $ & $ 3.4774 \pm 0.0045 $ \\
       HV 02538 & 13.8723 & 18.480 & $0.003 \pm 0.010 $ &  \nodata & $  0.926 \pm 0.002 $ & $ -0.036 \pm 0.004 $ & $ 2.2165 \pm 0.0029 $ \\
       HV 02339 & 13.8797 & 18.517 & $0.226 \pm 0.010 $ &  \nodata & $  0.895 \pm 0.002 $ & \phs $  0.047 \pm 0.004 $ & $ 3.5484 \pm 0.0048 $ \\
       HV 00911 & 13.9089 & 18.515 & $0.112 \pm 0.010 $ &  \nodata & $  0.884 \pm 0.002 $ & \phs $  0.017 \pm 0.004 $ & $ 4.3635 \pm 0.0042 $ \\
       HV 02463 & 13.9627 & 18.497 & $0.058 \pm 0.010 $ &  \nodata & $  0.909 \pm 0.002 $ & \phs $  0.011 \pm 0.004 $ & $ 4.2111 \pm 0.0048 $ \\
       HV 02244 & 13.9782 & 18.523 & $0.519 \pm 0.011 $ &  \nodata & $  0.802 \pm 0.003 $ & \phs $  0.160 \pm 0.004 $ & $ 4.4051 \pm 0.0051 $ \\
       HV 02647 & 14.1904 & 18.477 & $0.155 \pm 0.019 $ &  \nodata & $  0.853 \pm 0.003 $ & $ -0.017 \pm 0.006 $ & $ 3.1441 \pm 0.0037 $ \\
       HV 05655 & 14.2121 & 18.530 & $0.096 \pm 0.009 $ &  \nodata & $  0.896 \pm 0.002 $ & $ -0.005 \pm 0.003 $ & $ 3.9795 \pm 0.0050 $ \\
       HV 01006 & 14.2165 & 18.474 & $0.330 \pm 0.011 $ &  \nodata & $  0.865 \pm 0.002 $ & \phs $  0.074 \pm 0.004 $ & $ 4.7891 \pm 0.0061 $ \\
       HV 12505 & 14.3918 & 18.534 & $0.311 \pm 0.011 $ &  \nodata & $  0.857 \pm 0.002 $ & \phs $  0.043 \pm 0.004 $ & $ 4.1898 \pm 0.0063 $ \\
       HV 02324 & 14.4668 & 18.512 & $0.194 \pm 0.006 $ &  \nodata & $  0.883 \pm 0.001 $ & \phs $  0.037 \pm 0.002 $ & $ 4.1213 \pm 0.0054 $ \\
       HV 00887 & 14.4891 & 18.534 & $0.095 \pm 0.009 $ &  \nodata & $  0.921 \pm 0.002 $ & \phs $  0.019 \pm 0.003 $ & $ 4.2407 \pm 0.0054 $ \\
       HV 02282 & 14.6765 & 18.541 & $0.199 \pm 0.011 $ &  \nodata & $  0.896 \pm 0.002 $ & \phs $  0.038 \pm 0.004 $ & $ 4.4960 \pm 0.0058 $ \\
       HV 02356 & 15.1268 & 18.514 & $0.141 \pm 0.012 $ &  \nodata & $  0.879 \pm 0.002 $ & \phs $  0.033 \pm 0.004 $ & $ 5.0884 \pm 0.0059 $ \\
       HV 02249 & 15.2123 & 18.516 & $0.132 \pm 0.019 $ &  \nodata & $  0.865 \pm 0.003 $ & \phs $  0.055 \pm 0.006 $ & $ 5.2482 \pm 0.0086 $ \\
       HV 00933 & 15.5492 & 18.500 & $0.155 \pm 0.019 $ &  \nodata & $  0.894 \pm 0.003 $ & $ -0.014 \pm 0.006 $ & $ 5.8634 \pm 0.0053 $ \\
       HV 02262 & 15.8321 & 18.546 & $0.167 \pm 0.009 $ &  \nodata & $  0.948 \pm 0.002 $ & \phs $  0.018 \pm 0.003 $ & $ 4.2995 \pm 0.0055 $ \\
       HV 00973 & 15.8439 & 18.496 & $0.144 \pm 0.019 $ &  \nodata & $  0.919 \pm 0.003 $ & \phs $  0.031 \pm 0.006 $ & $ 5.4489 \pm 0.0048 $ \\
       HV 12471 & 15.8613 & 18.551 & $0.254 \pm 0.006 $ &  \nodata & $  0.913 \pm 0.001 $ & \phs $  0.016 \pm 0.002 $ & $ 3.9790 \pm 0.0046 $ \\
       HV 00892 & 15.9892 & 18.522 & $0.396 \pm 0.010 $ &  \nodata & $  0.849 \pm 0.002 $ & \phs $  0.114 \pm 0.004 $ & $ 6.0386 \pm 0.0060 $ \\
       HV 00985 & 15.9918 & 18.491 & $0.153 \pm 0.019 $ &  \nodata & $  0.914 \pm 0.002 $ & $ -0.005 \pm 0.006 $ & $ 4.7158 \pm 0.0042 $ \\
       HV 02772 & 16.1618 & 18.481 & $0.351 \pm 0.009 $ &  \nodata & $  0.937 \pm 0.001 $ & \phs $  0.021 \pm 0.003 $ & $ 5.8403 \pm 0.0064 $ \\
       HV 02549 & 16.2184 & 18.515 & $0.045 \pm 0.005 $ &  \nodata & $  0.976 \pm 0.001 $ & \phs $  0.012 \pm 0.002 $ & $ 4.6755 \pm 0.0054 $ \\
       HV 02273 & 16.8363 & 18.509 & $0.055 \pm 0.009 $ &  \nodata & $  0.879 \pm 0.001 $ & $ -0.002 \pm 0.003 $ & $ 4.6856 \pm 0.0053 $ \\
       HV 02580 & 16.9436 & 18.452 & $0.198 \pm 0.007 $ &  \nodata & $  0.938 \pm 0.001 $ & \phs $  0.045 \pm 0.002 $ & $ 3.7159 \pm 0.0042 $ \\
       HV 05594 & 17.2018 & 18.494 & $0.142 \pm 0.019 $ &  \nodata & $  0.896 \pm 0.003 $ & \phs $  0.018 \pm 0.006 $ & $ 5.0370 \pm 0.0062 $ \\
       HV 00891 & 17.2116 & 18.525 & $0.168 \pm 0.011 $ &  \nodata & $  0.935 \pm 0.002 $ & \phs $  0.053 \pm 0.004 $ & $ 5.5215 \pm 0.0078 $ \\
       HV 02261 & 17.2725 & 18.547 & $0.110 \pm 0.009 $ &  \nodata & $  1.071 \pm 0.001 $ & \phs $  0.006 \pm 0.003 $ & $ 4.9851 \pm 0.0062 $ \\
       HV 02319 & 17.4592 & 18.517 & $0.047 \pm 0.008 $ &  \nodata & $  0.970 \pm 0.001 $ & $ -0.021 \pm 0.003 $ & $ 4.5457 \pm 0.0052 $ \\
       HV 02288 & 17.5218 & 18.529 & $0.146 \pm 0.019 $ &  \nodata & $  0.948 \pm 0.003 $ & \phs $  0.019 \pm 0.006 $ & $ 4.9790 \pm 0.0064 $ \\
       HV 02791 & 17.7945 & 18.478 & $0.157 \pm 0.019 $ &  \nodata & $  0.922 \pm 0.003 $ & $ -0.027 \pm 0.006 $ & $ 5.1413 \pm 0.0053 $ \\
       HV 00901 & 18.4696 & 18.522 & $0.078 \pm 0.012 $ &  \nodata & $  0.976 \pm 0.003 $ & $ -0.026 \pm 0.005 $ & $ 4.8267 \pm 0.0066 $ \\
       HV 12499 & 18.4865 & 18.514 & $0.140 \pm 0.019 $ &  \nodata & $  0.946 \pm 0.003 $ & \phs $  0.031 \pm 0.006 $ & $ 2.4702 \pm 0.0038 $ \\
      OIII 1080 & 18.6617 & 18.515 & $0.155 \pm 0.019 $ &  \nodata & $  1.018 \pm 0.003 $ & \phs $  0.007 \pm 0.006 $ & $ 4.2241 \pm 0.0042 $ \\
       HV 01005 & 18.7147 & 18.469 & $0.243 \pm 0.006 $ &  \nodata & $  0.917 \pm 0.001 $ & \phs $  0.053 \pm 0.002 $ & $ 5.6540 \pm 0.0059 $ \\
       HV 02488 & 19.1631 & 18.496 & $0.150 \pm 0.012 $ &  \nodata & $  0.986 \pm 0.002 $ & \phs $  0.008 \pm 0.004 $ & $ 5.1324 \pm 0.0047 $ \\
       HV 02793 & 19.2186 & 18.458 & $0.097 \pm 0.005 $ &  \nodata & $  1.014 \pm 0.001 $ & $ -0.021 \pm 0.002 $ & $ 4.5000 \pm 0.0051 $ \\
        U 00011 & 20.0801 & 18.500 & $0.200 \pm 0.007 $ &  \nodata & $  0.980 \pm 0.002 $ & \phs $  0.034 \pm 0.002 $ & $ 4.4919 \pm 0.0081 $ \\
       HV 02789 & 20.3192 & 18.469 & $0.139 \pm 0.019 $ &  \nodata & $  0.919 \pm 0.003 $ & \phs $  0.011 \pm 0.006 $ & $ 4.4630 \pm 0.0060 $ \\
      OIII 0847 & 20.6393 & 18.524 & $0.151 \pm 0.019 $ &  \nodata & $  0.976 \pm 0.003 $ & $ -0.008 \pm 0.006 $ & $ 5.5741 \pm 0.0055 $ \\
       HV 00885 & 20.7032 & 18.528 & $0.367 \pm 0.011 $ &  \nodata & $  1.015 \pm 0.002 $ & \phs $  0.089 \pm 0.004 $ & $ 3.9984 \pm 0.0055 $ \\
       HV 00893 & 21.1169 & 18.523 & $0.146 \pm 0.005 $ &  \nodata & $  1.016 \pm 0.001 $ & \phs $  0.009 \pm 0.002 $ & $ 5.3500 \pm 0.0060 $ \\
       HV 02292 & 21.2628 & 18.528 & $0.143 \pm 0.019 $ &  \nodata & $  1.009 \pm 0.003 $ & \phs $  0.024 \pm 0.006 $ & $ 5.8784 \pm 0.0071 $ \\
       HV 02453 & 21.6093 & 18.505 & $0.147 \pm 0.019 $ &  \nodata & $  1.008 \pm 0.003 $ & \phs $  0.010 \pm 0.006 $ & $ 2.5051 \pm 0.0034 $ \\
       HV 02245 & 22.0882 & 18.548 & $0.148 \pm 0.019 $ &  \nodata & $  0.982 \pm 0.003 $ & $ -0.006 \pm 0.006 $ & $ 4.5856 \pm 0.0058 $ \\
       HV 02291 & 22.3170 & 18.524 & $0.020 \pm 0.010 $ &  \nodata & $  1.055 \pm 0.002 $ & $ -0.047 \pm 0.004 $ & $ 5.1448 \pm 0.0054 $ \\
      OIII 0079 & 22.5436 & 18.557 & $0.147 \pm 0.019 $ &  \nodata & $  1.002 \pm 0.003 $ & \phs $  0.001 \pm 0.006 $ & $ 5.7966 \pm 0.0072 $ \\
       HV 00876 & 22.7149 & 18.519 & $0.032 \pm 0.006 $ &  \nodata & $  1.057 \pm 0.001 $ & $ -0.016 \pm 0.002 $ & $ 5.8064 \pm 0.0066 $ \\
       HV 00984 & 23.0499 & 18.485 & $0.160 \pm 0.019 $ &  \nodata & $  1.087 \pm 0.002 $ & $ -0.013 \pm 0.006 $ & $ 4.7617 \pm 0.0039 $ \\
       HV 02755 & 23.1090 & 18.469 & $0.164 \pm 0.019 $ &  \nodata & $  1.034 \pm 0.003 $ & $ -0.048 \pm 0.006 $ & $ 3.3897 \pm 0.0048 $ \\
       HV 00878 & 23.3076 & 18.546 & $0.146 \pm 0.016 $ &  \nodata & $  1.034 \pm 0.004 $ & \phs $  0.032 \pm 0.006 $ & $ 6.4114 \pm 0.0116 $ \\
       HV 00886 & 23.9814 & 18.497 & $0.103 \pm 0.004 $ &  \nodata & $  1.081 \pm 0.001 $ & \phs $  0.015 \pm 0.002 $ & $ 6.7130 \pm 0.0059 $ \\
       HV 01013 & 24.1324 & 18.452 & $0.167 \pm 0.004 $ &  \nodata & $  1.074 \pm 0.001 $ & $ -0.006 \pm 0.002 $ & $ 4.9578 \pm 0.0055 $ \\
       HV 01003 & 24.3504 & 18.467 & $0.099 \pm 0.004 $ &  \nodata & $  1.071 \pm 0.001 $ & \phs $  0.027 \pm 0.002 $ & $ 5.7612 \pm 0.0056 $ \\
       HV 00889 & 25.8025 & 18.525 & $0.136 \pm 0.004 $ &  \nodata & $  1.106 \pm 0.001 $ & $ -0.008 \pm 0.002 $ & $ 4.8431 \pm 0.0047 $ \\
       HV 12815 & 26.1142 & 18.448 & $0.135 \pm 0.003 $ & \phs $  289.2 \pm 0.1 $ & $  1.104 \pm 0.001 $ & $ -0.002 \pm 0.002 $ & $ 6.2955 \pm 0.0046 $ \\
       HV 00902 & 26.3441 & 18.535 & $0.036 \pm 0.004 $ &  \nodata & $  1.101 \pm 0.001 $ & \phs $  0.003 \pm 0.002 $ & $ 6.4356 \pm 0.0069 $ \\
       HV 01023 & 26.5551 & 18.444 & $0.115 \pm 0.005 $ &  \nodata & $  1.074 \pm 0.001 $ & $ -0.015 \pm 0.002 $ & $ 5.9098 \pm 0.0083 $ \\
       HV 02251 & 27.9009 & 18.505 & $0.122 \pm 0.005 $ &  \nodata & $  1.121 \pm 0.001 $ & \phs $  0.014 \pm 0.002 $ & $ 7.0488 \pm 0.0108 $ \\
       HV 02540 & 28.1037 & 18.497 & $0.139 \pm 0.019 $ &  \nodata & $  1.046 \pm 0.003 $ & \phs $  0.014 \pm 0.006 $ & $ 7.3314 \pm 0.0097 $ \\
       HV 00934 & 28.1934 & 18.486 & $0.201 \pm 0.013 $ &  \nodata & $  1.117 \pm 0.003 $ & $ -0.027 \pm 0.003 $ & $ 6.1843 \pm 0.0132 $ \\
       HV 08036 & 28.3740 & 18.570 & $0.081 \pm 0.006 $ &  \nodata & $  1.115 \pm 0.002 $ & $ -0.017 \pm 0.002 $ & $ 7.0218 \pm 0.0118 $ \\
       HV 00904 & 30.4018 & 18.515 & $0.229 \pm 0.010 $ &  \nodata & $  1.101 \pm 0.002 $ & \phs $  0.033 \pm 0.003 $ & $ 6.5932 \pm 0.0069 $ \\
       HV 00875 & 30.4136 & 18.542 & $0.100 \pm 0.005 $ &  \nodata & $  1.118 \pm 0.001 $ & \phs $  0.031 \pm 0.002 $ & $ 3.1626 \pm 0.0060 $ \\
       HV 01002 & 30.4761 & 18.446 & $0.070 \pm 0.004 $ &  \nodata & $  1.139 \pm 0.001 $ & \phs $  0.010 \pm 0.002 $ & $ 6.5630 \pm 0.0059 $ \\
       HV 00899 & 31.0511 & 18.519 & $0.043 \pm 0.005 $ & \phs $  272.3 \pm 0.1 $ & $  1.142 \pm 0.001 $ & $ -0.028 \pm 0.002 $ & $ 6.9025 \pm 0.0050 $ \\
       HV 00882 & 31.7907 & 18.538 & $0.175 \pm 0.004 $ &  \nodata & $  1.135 \pm 0.001 $ & \phs $  0.011 \pm 0.002 $ & $ 6.2635 \pm 0.0082 $ \\
       HV 00873 & 34.4359 & 18.562 & $0.065 \pm 0.005 $ &  \nodata & $  1.204 \pm 0.001 $ & $ -0.018 \pm 0.002 $ & $ 5.7279 \pm 0.0095 $ \\
       HV 00881 & 35.7411 & 18.549 & $0.054 \pm 0.005 $ &  \nodata & $  1.193 \pm 0.001 $ & $ -0.019 \pm 0.002 $ & $ 6.2447 \pm 0.0079 $ \\
       HV 02294 & 36.5447 & 18.496 & $0.097 \pm 0.003 $ &  \nodata & $  1.218 \pm 0.001 $ & \phs $  0.008 \pm 0.002 $ & $ 6.3331 \pm 0.0050 $ \\
       HV 00879 & 36.8299 & 18.540 & $0.117 \pm 0.004 $ & \phs $  252.7 \pm 0.0 $ & $  1.192 \pm 0.001 $ & $ -0.022 \pm 0.002 $ & $ 6.2112 \pm 0.0046 $ \\
       HV 00909 & 37.5563 & 18.532 & $0.036 \pm 0.004 $ & \phs $  237.6 \pm 0.0 $ & $  1.194 \pm 0.001 $ & \phs $  0.002 \pm 0.002 $ & $ 5.2002 \pm 0.0037 $ \\
       HV 02338 & 42.1904 & 18.546 & $0.052 \pm 0.004 $ & \phs $  244.4 \pm 0.0 $ & $  1.260 \pm 0.001 $ & $ -0.020 \pm 0.002 $ & $ 6.2748 \pm 0.0045 $ \\
       HV 00877 & 45.1563 & 18.526 & $0.087 \pm 0.004 $ &  \nodata & $  1.254 \pm 0.001 $ & $ -0.053 \pm 0.002 $ & $ 3.8424 \pm 0.0035 $ \\
       HV 00953 & 48.0796 & 18.475 & $0.108 \pm 0.004 $ &  \nodata & $  1.303 \pm 0.001 $ & \phs $  0.010 \pm 0.002 $ & $ 5.4350 \pm 0.0052 $ \\
       HV 02369 & 48.4003 & 18.487 & $0.161 \pm 0.003 $ &  \nodata & $  1.293 \pm 0.001 $ & \phs $  0.000 \pm 0.002 $ & $ 6.2752 \pm 0.0059 $ \\
       HV 02827 & 78.8038 & 18.432 & $0.108 \pm 0.003 $ & \phs $  301.5 \pm 0.1 $ & $  1.427 \pm 0.001 $ & $ -0.042 \pm 0.002 $ & $ 3.9088 \pm 0.0040 $ \\
       HV 05497 & 99.6143 & 18.512 & $0.065 \pm 0.004 $ & \phs $  287.2 \pm 0.1 $ & $  1.523 \pm 0.001 $ & $ -0.053 \pm 0.002 $ & $ 3.6828 \pm 0.0069 $ \\
\enddata


==> smc.tex <==
\tablehead{ 
\colhead{Name} & \colhead {$ P$ [d]} & \colhead{$\mu$ [mag]} & \colhead{$E(B-V)$ [mag]} & \colhead{$\bar{v}$ [km s$^{-1}$]} & \colhead{$ \bar{\rho} $} & \colhead{$\bar{\tau}$} & \colhead{$ A^2 \times 10^2$}}
\startdata
       HV 06320 & 10.0998 & $19.017 \pm 0.071 $ & $0.148 \pm 0.015 $ &  \nodata & $  0.757 \pm 0.014 $ & \phs $  0.078 \pm 0.004 $ & $ 3.7284 \pm 0.0095 $ \\
       HV 02063 & 11.1663 & $18.881 \pm 0.071 $ & $0.167 \pm 0.007 $ &  \nodata & $  0.815 \pm 0.014 $ & \phs $  0.055 \pm 0.002 $ & $ 2.8573 \pm 0.0033 $ \\
       HV 02017 & 11.4091 & $18.870 \pm 0.071 $ & $0.175 \pm 0.007 $ &  \nodata & $  0.823 \pm 0.014 $ & \phs $  0.060 \pm 0.002 $ & $ 3.0375 \pm 0.0030 $ \\
       HV 01610 & 11.6431 & $18.944 \pm 0.071 $ & $0.171 \pm 0.009 $ &  \nodata & $  0.814 \pm 0.014 $ & \phs $  0.070 \pm 0.003 $ & $ 3.7982 \pm 0.0038 $ \\
       HV 00856 & 12.1557 & $19.038 \pm 0.071 $ & $0.273 \pm 0.008 $ &  \nodata & $  0.809 \pm 0.014 $ & \phs $  0.081 \pm 0.003 $ & $ 3.6536 \pm 0.0043 $ \\
       HV 01365 & 12.4127 & $19.483 \pm 0.016 $ & $0.231 \pm 0.005 $ & \phs $  126.8 \pm 0.1 $ & $  0.885 \pm 0.003 $ & \phs $  0.070 \pm 0.002 $ & $ 3.3213 \pm 0.0026 $ \\
       HV 02227 & 12.4663 & $18.866 \pm 0.071 $ & $0.201 \pm 0.010 $ &  \nodata & $  0.851 \pm 0.014 $ & \phs $  0.048 \pm 0.003 $ & $ 3.3765 \pm 0.0036 $ \\
       HV 02230 & 12.5294 & $18.823 \pm 0.071 $ & $0.218 \pm 0.010 $ &  \nodata & $  0.861 \pm 0.014 $ & \phs $  0.051 \pm 0.003 $ & $ 3.0924 \pm 0.0067 $ \\
       HV 02052 & 12.5778 & $18.858 \pm 0.071 $ & $0.084 \pm 0.008 $ &  \nodata & $  0.855 \pm 0.014 $ & \phs $  0.058 \pm 0.003 $ & $ 3.8876 \pm 0.0045 $ \\
       HV 01744 & 12.6237 & $18.925 \pm 0.071 $ & $0.135 \pm 0.009 $ & \phs $  141.9 \pm 5.8 $ & $  0.842 \pm 0.014 $ & \phs $  0.061 \pm 0.003 $ & $ 4.0334 \pm 0.0046 $ \\
       HV 01873 & 12.9396 & $19.026 \pm 0.071 $ & $0.185 \pm 0.007 $ &  \nodata & $  0.830 \pm 0.014 $ & \phs $  0.060 \pm 0.002 $ & $ 4.4509 \pm 0.0041 $ \\
       HV 02225 & 13.1477 & $18.877 \pm 0.071 $ & $0.119 \pm 0.014 $ &  \nodata & $  0.865 \pm 0.014 $ & \phs $  0.024 \pm 0.004 $ & $ 3.5367 \pm 0.0095 $ \\
       HV 02202 & 13.1921 & $18.852 \pm 0.071 $ & $0.227 \pm 0.008 $ &  \nodata & $  0.871 \pm 0.014 $ & \phs $  0.073 \pm 0.002 $ & $ 3.7139 \pm 0.0051 $ \\
       HV 00827 & 13.4642 & $18.935 \pm 0.071 $ & $0.186 \pm 0.006 $ &  \nodata & $  0.861 \pm 0.014 $ & \phs $  0.072 \pm 0.002 $ & $ 3.6416 \pm 0.0031 $ \\
       HV 02189 & 13.4703 & $18.989 \pm 0.071 $ & $0.360 \pm 0.022 $ &  \nodata & $  0.850 \pm 0.014 $ & \phs $  0.114 \pm 0.007 $ & $ 3.5912 \pm 0.0039 $ \\
       HV 01326 & 13.7250 & $19.041 \pm 0.071 $ & $0.169 \pm 0.009 $ &  \nodata & $  0.845 \pm 0.014 $ & \phs $  0.049 \pm 0.003 $ & $ 3.4243 \pm 0.0033 $ \\
       HV 01335 & 14.3814 & $19.079 \pm 0.071 $ & $0.243 \pm 0.009 $ &  \nodata & $  0.852 \pm 0.014 $ & \phs $  0.076 \pm 0.003 $ & $ 3.5012 \pm 0.0039 $ \\
       HV 02088 & 14.5796 & $18.955 \pm 0.071 $ & $0.208 \pm 0.008 $ &  \nodata & $  0.881 \pm 0.014 $ & \phs $  0.052 \pm 0.002 $ & $ 4.4474 \pm 0.0053 $ \\
       HV 00843 & 14.7136 & $18.927 \pm 0.071 $ & $0.120 \pm 0.009 $ & \phs $  166.8 \pm 5.8 $ & $  0.888 \pm 0.014 $ & \phs $  0.002 \pm 0.003 $ & $ 4.1825 \pm 0.0037 $ \\
       HV 02233 & 15.1677 & $18.807 \pm 0.071 $ & $0.271 \pm 0.016 $ &  \nodata & $  0.922 \pm 0.014 $ & \phs $  0.102 \pm 0.004 $ & $ 5.0158 \pm 0.0141 $ \\
       HV 01442 & 15.2886 & $18.964 \pm 0.071 $ & $0.232 \pm 0.006 $ & \phs $  130.0 \pm 7.1 $ & $  0.893 \pm 0.014 $ & \phs $  0.046 \pm 0.002 $ & $ 4.4427 \pm 0.0041 $ \\
       HV 01560 & 15.5099 & $18.845 \pm 0.071 $ & $-0.023 \pm 0.007 $ & \phs $  109.4 \pm 5.0 $ & $  0.921 \pm 0.014 $ & $ -0.034 \pm 0.002 $ & $ 4.2721 \pm 0.0035 $ \\
       HV 01482 & 15.8233 & $18.996 \pm 0.071 $ & $0.286 \pm 0.007 $ & \phs $  137.0 \pm 7.1 $ & $  0.897 \pm 0.014 $ & \phs $  0.060 \pm 0.002 $ & $ 4.8315 \pm 0.0040 $ \\
       HV 01328 & 15.8372 & $18.985 \pm 0.071 $ & $0.115 \pm 0.006 $ &  \nodata & $  0.900 \pm 0.014 $ & \phs $  0.069 \pm 0.002 $ & $ 3.3624 \pm 0.0032 $ \\
       HV 00854 & 15.9594 & $18.948 \pm 0.071 $ & $0.119 \pm 0.008 $ &  \nodata & $  0.909 \pm 0.014 $ & \phs $  0.049 \pm 0.003 $ & $ 5.0430 \pm 0.0046 $ \\
       HV 01787 & 16.1929 & $18.919 \pm 0.071 $ & $0.202 \pm 0.010 $ & \phs $  166.1 \pm 5.8 $ & $  0.920 \pm 0.014 $ & \phs $  0.060 \pm 0.003 $ & $ 4.6634 \pm 0.0050 $ \\
       HV 01954 & 16.6948 & $18.842 \pm 0.071 $ & $0.230 \pm 0.004 $ &  \nodata & $  0.944 \pm 0.014 $ & \phs $  0.083 \pm 0.002 $ & $ 3.4538 \pm 0.0027 $ \\
       HV 00822 & 16.7420 & $18.953 \pm 0.071 $ & $0.114 \pm 0.006 $ &  \nodata & $  0.923 \pm 0.014 $ & \phs $  0.023 \pm 0.002 $ & $ 5.2660 \pm 0.0040 $ \\
       HV 01925 & 17.1997 & $19.051 \pm 0.071 $ & $0.064 \pm 0.006 $ &  \nodata & $  0.911 \pm 0.014 $ & \phs $  0.061 \pm 0.002 $ & $ 3.3039 \pm 0.0030 $ \\
       HV 01342 & 17.9409 & $19.037 \pm 0.071 $ & $0.119 \pm 0.004 $ &  \nodata & $  0.927 \pm 0.014 $ & \phs $  0.059 \pm 0.002 $ & $ 2.2636 \pm 0.0018 $ \\
       HV 01884 & 18.1102 & $18.919 \pm 0.071 $ & $0.065 \pm 0.007 $ & \phs $  160.8 \pm 5.8 $ & $  0.952 \pm 0.014 $ & \phs $  0.002 \pm 0.002 $ & $ 3.9278 \pm 0.0032 $ \\
       HV 00817 & 18.9004 & $18.899 \pm 0.071 $ & $0.174 \pm 0.005 $ &  \nodata & $  0.970 \pm 0.014 $ & \phs $  0.069 \pm 0.002 $ & $ 4.1861 \pm 0.0033 $ \\
       HV 01543 & 20.4547 & $19.029 \pm 0.071 $ & $0.334 \pm 0.007 $ & \phs $  172.6 \pm 7.1 $ & $  0.969 \pm 0.014 $ & \phs $  0.060 \pm 0.002 $ & $ 4.8772 \pm 0.0043 $ \\
       HV 11211 & 21.3856 & $18.778 \pm 0.071 $ & $0.149 \pm 0.007 $ &  \nodata & $  1.032 \pm 0.014 $ & \phs $  0.031 \pm 0.002 $ & $ 4.9987 \pm 0.0073 $ \\
       HV 01522 & 22.1495 & $19.032 \pm 0.071 $ & $0.130 \pm 0.006 $ & \phs $  162.8 \pm 10.0 $ & $  0.992 \pm 0.014 $ & \phs $  0.017 \pm 0.002 $ & $ 5.1628 \pm 0.0044 $ \\
       HV 02209 & 22.6431 & $18.827 \pm 0.071 $ & $0.137 \pm 0.004 $ &  \nodata & $  1.040 \pm 0.014 $ & \phs $  0.054 \pm 0.002 $ & $ 3.2634 \pm 0.0030 $ \\
       HV 01430 & 23.9688 & $19.073 \pm 0.071 $ & $0.195 \pm 0.008 $ & \phs $  126.8 \pm 7.1 $ & $  1.008 \pm 0.014 $ & \phs $  0.039 \pm 0.003 $ & $ 5.5388 \pm 0.0044 $ \\
       HV 02205 & 25.4280 & $18.880 \pm 0.071 $ & $0.231 \pm 0.009 $ &  \nodata & $  1.064 \pm 0.014 $ & \phs $  0.030 \pm 0.003 $ & $ 5.2193 \pm 0.0057 $ \\
       HV 00847 & 27.0773 & $18.980 \pm 0.071 $ & $0.210 \pm 0.005 $ &  \nodata & $  1.063 \pm 0.014 $ & \phs $  0.042 \pm 0.002 $ & $ 5.3974 \pm 0.0042 $ \\
       HV 00819 & 28.4428 & $18.974 \pm 0.071 $ & $0.235 \pm 0.005 $ &  \nodata & $  1.079 \pm 0.014 $ & \phs $  0.030 \pm 0.002 $ & $ 5.9630 \pm 0.0058 $ \\
       HV 00863 & 28.9732 & $18.829 \pm 0.071 $ & $0.210 \pm 0.007 $ &  \nodata & $  1.114 \pm 0.014 $ & \phs $  0.054 \pm 0.002 $ & $ 6.7360 \pm 0.0116 $ \\
       HV 01451 & 30.0729 & $18.871 \pm 0.071 $ & $0.145 \pm 0.006 $ & \phs $  138.1 \pm 7.1 $ & $  1.118 \pm 0.014 $ & $ -0.009 \pm 0.002 $ & $ 4.7977 \pm 0.0037 $ \\
       HV 00823 & 31.9260 & $18.837 \pm 0.071 $ & $0.127 \pm 0.004 $ &  \nodata & $  1.142 \pm 0.014 $ & $ -0.004 \pm 0.002 $ & $ 5.4921 \pm 0.0046 $ \\
       HV 01636 & 32.7350 & $19.149 \pm 0.071 $ & $0.809 \pm 0.011 $ &  \nodata & $  1.087 \pm 0.014 $ & \phs $  0.200 \pm 0.003 $ & $ 4.7947 \pm 0.0041 $ \\
       HV 00840 & 33.0323 & $18.913 \pm 0.071 $ & $0.112 \pm 0.005 $ & \phs $  164.1 \pm 5.8 $ & $  1.137 \pm 0.014 $ & \phs $  0.010 \pm 0.002 $ & $ 6.5207 \pm 0.0054 $ \\
       HV 00865 & 33.3617 & $18.860 \pm 0.071 $ & $0.217 \pm 0.007 $ &  \nodata & $  1.150 \pm 0.014 $ & \phs $  0.063 \pm 0.002 $ & $ 5.7490 \pm 0.0095 $ \\
       HV 02064 & 33.6635 & $18.961 \pm 0.071 $ & $0.150 \pm 0.004 $ &  \nodata & $  1.133 \pm 0.014 $ & \phs $  0.013 \pm 0.002 $ & $ 5.3226 \pm 0.0042 $ \\
       HV 02231 & 36.6861 & $18.866 \pm 0.071 $ & $0.166 \pm 0.008 $ &  \nodata & $  1.178 \pm 0.014 $ & \phs $  0.008 \pm 0.003 $ & $ 5.1925 \pm 0.0074 $ \\
       HV 11182 & 39.1905 & $18.942 \pm 0.071 $ & $0.137 \pm 0.004 $ & \phs $  146.0 \pm 5.8 $ & $  1.183 \pm 0.014 $ & $ -0.007 \pm 0.002 $ & $ 3.8103 \pm 0.0036 $ \\
       HV 02195 & 41.8100 & $18.877 \pm 0.071 $ & $0.076 \pm 0.004 $ &  \nodata & $  1.215 \pm 0.014 $ & \phs $  0.014 \pm 0.002 $ & $ 4.6342 \pm 0.0042 $ \\
       HV 01877 & 49.7343 & $18.922 \pm 0.071 $ & $0.330 \pm 0.005 $ & \phs $  201.1 \pm 5.8 $ & $  1.259 \pm 0.014 $ & \phs $  0.050 \pm 0.002 $ & $ 4.1826 \pm 0.0044 $ \\
       HV 00824 & 65.8331 & $19.102 \pm 0.021 $ & $0.165 \pm 0.004 $ & \phs $  139.6 \pm 0.1 $ & $  1.400 \pm 0.004 $ & \phs $  0.031 \pm 0.002 $ & $ 5.6361 \pm 0.0100 $ \\
       HV 11157 & 69.0304 & $18.937 \pm 0.071 $ & $0.152 \pm 0.004 $ &  \nodata & $  1.355 \pm 0.014 $ & $ -0.009 \pm 0.002 $ & $ 2.6402 \pm 0.0039 $ \\
\enddata

